A Comprehensive Survey of Multilingual Neural Machine Translation

We present a survey on multilingual neural machine translation (MNMT), which has gained a lot of traction in the recent years. MNMT has been useful in improving translation quality as a result of translation knowledge transfer (transfer learning). MNMT is more promising and interesting than its statistical machine translation counterpart because end-to-end modeling and distributed representations open new avenues for research on machine translation. Many approaches have been proposed in order to exploit multilingual parallel corpora for improving translation quality. However, the lack of a comprehensive survey makes it difficult to determine which approaches are promising and hence deserve further exploration. In this paper, we present an in-depth survey of existing literature on MNMT. We first categorize various approaches based on their central use-case and then further categorize them based on resource scenarios, underlying modeling principles, core-issues and challenges. Wherever possible we address the strengths and weaknesses of several techniques by comparing them with each other. We also discuss the future directions that MNMT research might take. This paper is aimed towards both, beginners and experts in NMT. We hope this paper will serve as a starting point as well as a source of new ideas for researchers and engineers interested in MNMT.

==> auxiliary.tex <==
% \subsection{One Model for Many to Many Translation}
% \citet{P15-1166} proposed the first multilingual model for one to many NMT and trained this model by {\it multi-task learning}. In this model there is a single shared encoder for the only source language and separate decoders for each target language. The attention mechanism is separate for each target language. 
% % This one to many model was able to leverage the abundance of the source language corpora and learn better encodings for input sentences leading to a substantial improvement in translation quality. Furthermore, multi-task learning has a regularization effect during training which also contributed to the improvement in translation quality. 
% \citet{Q17-1026} proposed a many-to-one NMT model and alleviated the problem of large multilingual vocabularies by resorting to character level processing. They showed that a single encoder can be shared between multiple source languages and this many-to-one model can outperform a one-to-one model.
% One-to-many and many-to-one models were unified by \citet{N16-1101} who proposed a multilingual multiway model which could translate from $M$ source languages to $N$ target languages. The proposed model has multiple encoders and decoders one for each language but a shared attention mechanism.
% % The proposed model was a rather simple extension of the encoder-decoder model where multiple encoders and decoders, one for each language, were coupled using a shared attention mechanism. This model would later be used for multi-source and zero resource NMT (see Section \ref{sec:pivoting}). The most attractive feature of this MNMT model was that it could leverage the abundance of English as a language and improve the translation into English for all involved source languages. However, this way of MNMT modeling leads to a parameter explosion which sparked interest in research into reducing the size of MNMT models while maintaining quality. 
% However, this model is unable to translate between language pairs which have no training data. Another limitation of this model is that the burden of coupling multiple encoders and decoders falls on the shared attention mechanism which minimizes the possibility of generating language independent or universal representations for sentences. 
% Most of these limitations were addressed by \citet{johnson17} who proposed a MNMT model which uses the vanilla NMT model as a black-box and thus is a MNMT model where all parameters, except embeddings, are shared among multiple languages. Since this model also enables zero shot translation we cover it in Section \ref{sec:zeroshot}. \citet{N16-1101} and \citet{johnson17} are two extremes with regards to parameter sharing and have led to studies that explore parameter sharing strategies.

% Instead of sharing an attention mechanism between all decoders as om \citet{N16-1101}, \citet{DBLP:journals/corr/abs-1811-00498} propose to first transform language specific sentence embeddings into {\it universal sentence embeddings} which are then fed to a specific decoder that has its own attention mechanism. Each encoder and decoder has its own independent parameters, however the output of each encoder is processed by an ``attention bridge'' which is a self attention layer that is shared among all encoders. This process reduces the burden on the attention mechanisms and leads to better translation performance. On the other hand, \citet{C18-1263} propose a simple modification to \citet{johnson17} by augmenting the model input. Note that \citet{johnson17} proposed to translate into a target language by specifying the target language as a token which is appended to the source sentence. \citet{C18-1263} show that the shared attention mechanism is source language agnostic and is unable to leverage language specific information while computing context. As such, they propose to augment the source sentences with additional tokens which specify not only the target language but also the source language. This results in better attention leading to improvements in translation quality, even for the zero shot languages. \FIXME{This should probably go into the zero shot section.}

% Due to lack in clarity regarding what parts of the model should or should not be shared, \citet{W18-6327} conducted an empirical investigation of {\it parameter sharing} between decoders for one to many translation. In particular, they show that completely sharing all parameters as in \citet{johnson17} is effective when the target languages are linguistically similar. On the other hand, they showed that for linguistically dissimilar languages, sharing parameters between some parts of the decoders leads to optimal translation quality. Due to the exponential number of combinations of parameter sets that can be shared, \citet{W18-6327} only explored a fraction of the sharing configurations which does prove that further studies into what is shareable and what isn't is needed.  \citet{D18-1326} showed that explicitly reserving parts of the embedding vectors for specific languages helps generate better language specific representations for one to many translation. This suggests that a balance of sharing and separating representations is crucial for optimal translation quality in a multilingual scenario. On the other hand, \citet{D18-1039} improved upon \citet{C18-1263} to generate parameters on the fly for different language pairs. In essence, \citet{D18-1039} used linear transformations to convert a base set of parameters into language specific parameters for the encoder and the decoder. As a result, this contextual parameter generated model can simulate $NxM$ times the number of parameters as the one proposed in \citet{C18-1263} although it has only a small number of parameters needed by the contextual parameter generator. The result of contextual parameter generation is a large improvement in translation quality for both, seen and unseen language pairs. Another way of generating contextual generations is explored by \citet{N18-1032} who propose a Universal NMT model in which they generate language specific vocabulary representations from a universal set of shared tokens and interpolate embeddings for unseen tokens. They also use a single encoder and decoder to be shared between multiple languages but the encoder and decoder are composed of a mixture of language experts which is essentially mixture of experts \FIXME{Cite mixture of experts} that capture different features for different languages and thereby generate better representations in a multilingual scenario. 

% The lesson to be learned here is that parameter sharing is invaluable for making translation models compact, however too much parameter sharing could be detrimental and thus empirically determining the optimal parameter sharing strategy and contextualization of parameters depending on the languages involved is important.

% \subsection{Exploiting Multilingual Redundancy}
% A many-to-one translation scenario is one where one wishes to train a single model to translate from one of multiple source languages to a target language. It is known that some languages are harder to translate than others \FIXME{citation is needed here}, however it is also the case that there are linguistic phenomenon in one language that might be easier to translate when compared to another language \FIXME{need some citation if available}. For example: French to English translation is easier than German to English translation \FIXME{may submit WMT share task overview papers for this. why is needed, can be lexical and grammatical similarity}, however English is in the same language family as German. As such, if the same source sentence can be expressed in different languages then both sentences can be used together to improve the translation into English. This technique is known as multi-source machine translation \FIXME{citation} and is a special case of multi-modal translation \FIXME{cite multimodal works}\FIXME{i do not think it is a good idea to mention mutlimodal MT here, we do not have plans to compare multilingual to multmodal MT in this paper, right?}. In this case the underlying principle is to leverage redundancy \FIXME{what kind of? RAJ: Read the whole sentence} in terms of source side linguistic phenomena expressed in multiple languages. 

% Work on Multi-source SMT \FIXME{cite the work by Och and Ney in 2001 or 2003; I dont remember the exact year} has proven that the same source sentence in multiple languages can help improve translation quality. The very first work that proposed the multi-source NMT model focused on French+German to English translation \cite{N16-1004}. In this work, {\it separate encoders and attention mechanisms} were used for each source language. Once context representations are generated for each source language, they are combined in the decoder and this combination results in better target side context representations, leading to a substantial improvement in translation quality. Since, this approach requires multiple encoders and decoders, a simpler approach was proposed by \citet{Dabre-MTS2017} where the multiple {\it source sentences were concatenated} and fed to a standard NMT model. Surprisingly, this multi-source model was able to automatically identify the boundaries between different source languages and simplify the training process for multi-source NMT. \citet{Dabre-MTS2017} also showed that it is better to use linguistically similar source languages, especially in low-resource scenarios. Other ways to perform multi-source NMT involve {\it ensembling} of unidirectional \FIXME{The paper on learning an ensemble function for multi-source NMT. Published in coling 2016} or multilingual models \FIXME{Firats zero resource work; add citation here. Firats's work has been cited in all use cases, which is a little bit confusing..}. 

% All these works assume that during testing, the same sentence is available in multiple languages, which is rather impractical. As such, two additional works address the possibility of {\it missing source sentences}. The first of these works, proposed by \citet{choi2018improving} essentially extends \cite{N16-1004} by modifying the training data. The N-lingual corpora are used as in the original work. In addition bilingual corpora are converted into N-lingual corpora by representing each ``missing'' source language with a {\it dummy token}. As a result, the model is able to use an arbitrary number of sources languages for translation. \citet{nishimura18iwslt} further proposed to use {\it synthetic sentences}, obtained using translation, instead of a dummy token for the missing source languages. In essence, they generate a pseudo N-lingual corpus from several bilingual corpora and then train a multi-source NMT model using the method proposed by \citet{N16-1004}. Both these works are highly practical and help improve translation quality by a significant amount, although \cite{nishimura18iwslt} is more time consuming because multiple source sentences need to be generated in the case that they are missing. \FIXME{it is better to change the paragraph here}Multi-source NMT has also been used for post-editing where the translated sentence is used as an additional source, an idea that has shown to yield improvements without needing an N-lingual corpus. \FIXME{This work is by someone from NTT labs with Maasaki Nagata.}\FIXME{citation} \alertAK{Anoop: This usecase can be mentioned as a motivation from multi-source NMT at the beginning of the multisource section.}

% Approaches for multi-source NMT can be extremely useful for creating N-lingual corpora such as Europarl and UN. Instead of having a translator translate from scratch, multi-source NMT can be used to generate high quality translations which can then be post-edited, a process that is less labor intensive and cheaper compared to translating from scratch.

% \subsubsection{Pivoting} \label{sec:pivoting}
% Zero resource NMT was first explored by \citet{N16-1101} where a multilingual multiway NMT model \cite{N16-1004} was used to translate from Spanish to French using English as a pivot language. This pivoting was done either at run time or during pre-training. {\it Run-time pivoting} involved using the MNMT model to first translate from French to English and then from English to Spanish. Using the intermediate English translation as an additional source for multi-source translation \FIXME{see section on multisource NMT} was rather ineffective \FIXME{which work did this?}. As a MNMT model is known to give better English translations as compared to a model trained for a single translation direction, such pivoting can certainly lead to better translation quality as compared to the translations given by pivoting using two unidirectional models. Pivoting unidirectional models can be improved if they are jointly trained as shown by \citet{ijcai2017-555}. {\it Joint training} was achieved by either forcing the pivot language's parameters to be similar or by forcing the models to learn effective pivot language translations. The latter approach requires a small source-target parallel corpus and hence is not truly zero resource. However, both approaches are multilingual because of the coupling of the parameters of the otherwise independent models.

% {\it Pivoting during pre-training} involved using the MNMT model to first translate the Spanish side of the training corpus to English which in turn is translated into French. This gives a pseudo-parallel French-Spanish corpus where the source is synthetic and the target is original. The MNMT model is {\it fine tuned on this synthetic data} and this enables direct French to Spanish translation. This work \cite{N16-1101} also showed that a small clean parallel corpus between French and Spanish can be used for fine tuning and can have the same effect as a pseduo-parallel corpus which is two orders of magnitude larger.

% The approaches proposed so far involve pivoting or synthetic corpus generation which is a slow process due to its two step nature. As such, it is more interesting, and challenging, to enable translation between a zero resource pair without explicitly involving a pivot language during decoding or for generating pseudo-parallel corpora. This process of directly training a NMT model for a zero resource pair is known as zero shot NMT. Zero shot NMT also requires a pivot language but it is only used during training without the need for generating pseudo-parallel corpora.

% \subsubsection{Zero Shot} \label{sec:zeroshot}
% Zero Shot NMT was first shown to be possible by \citet{johnson17}  by sharing all model parameters for multiple languages. For each language direction, {\it a language tag} such as $<2tgt>$\footnote{The token \textit{tgt} can be the language code.} was appended to the source sentence, which in turn enabled the decoder to learn to translate into a specific target language. Due to complete {\it parameter sharing}, the encoder and decoder learn to generate a universal representation because of which it was possible to translate between a language pair which was never seen during training. Furthermore, fine tuning using a small parallel corpus was shown to outperform a model trained from scratch using a much larger parallel corpus. A similar work by \citet{DBLP:journals/corr/HaNW16} relied on appending target language tokens per source word but is essentially the same as \citet{johnson17}. However, work on translation for Indian languages \cite{Giulia-MTS2017} showed that zero shot works well only when the training corpora are extremely large. As the corpora for most Indian languages contain fewer than 100,000 lines the zero shot approach is rather infeasible despite linguistic similarity. \citet{DBLP:journals/corr/abs-1811-01389} confirmed this in the case of European languages where small training corpora were used. However, they used the zero shot approach by \citet{johnson17} to iteratively {\it generate pseudo-parallel corpora} for the zero resource language pair and added this data to the training data. This iterative process was shown to improve performance by over 10 BLEU compared to the naive zero shot performance. Note that this way of generating pseudo-parallel corpora is not possible using the MNMT model proposed by \citet{N16-1004} as it is unable to perform zero shot translation.

% Zero shot NMT models trained in this fashion tends to translate into the wrong language at times and \citet{DBLP:journals/corr/abs-1711-07893} proposed to {\it filter the output} of the softmax so as to force the model to translate into the desired language. They further proposed to incorporate linguistic information such as part-of-speech and morphological features for a {\it factored representation} of the input sentences which led to a further improvement in translation quality. Another important point is that it is better to incorporate multiple translation directions, including redundant directions such as English to English, to improve zero shot translation quality.

% This initial success in Zero Shot NMT motivated more sophisticated mechanisms which have advanced the state-of-art for underresourced languages. {\it Teacher-Student learning} was proposed by \citet{P17-1176} where they first trained a pivot-target NMT model and used it as a teacher to guide the behaviour of a source-target NMT model. The underlying assumption was that using a source-pivot sentence pair, the probability distribution for source-target translation should be close ot the pivot-target translation. As such, the pivot-target model can be used to provide the probability distribution for the target language and the source-target model can be trained by minimizing the KL divergence between the two distributions. The divergence can be computed at the sequence level or at the word level where the latter is shown to be superior.

% The teacher-student method was used in a multi-model fashion by \citet{DBLP:conf/aaai/ChenLL18} where the teacher model is an image captioning model which learns to caption an image into the source language and the student model is the source to target NMT model. The NMT model translates the generated captions into the target language and the translation rewards are obtained using a language model for the target language because source-target parallel corpora are not available. Translation rewarding falls in the realm of reinforcement learning which is known to work well for a number of unsupervised tasks \FIXME{Can anyone cite the works of openAI and deepmind for Go, Chess and DOTA? I think its relevant to mention this.}. While its possible to pre-train the captioning model and only train the NMT model, jointly learning both models is shown to yield superior results. Although joint training is more expensive, it shows that a teacher model also needs to adapt to the student model for the best possible results. This has parallels in real life where teachers have to adapt their teaching strategies depending on their students.

% {\it Reinforcement learning} for zero-shot learning was explored by \citet{DBLP:journals/corr/abs-1805-10338} where the dual learning framework was combined with rewards from language models. They initially train a single zero-shot model for source-target and target-source translation using source-pivot and pivot-target corpora. This initial model which is almost identical to \citet{johnson17} is then used for dual learning. Using small monolingual corpora for the zero shot languages, translations zero shot translation into the target language is performed followed by reconstruction by back-translating into the original language. Rewards for both the translations and the reconstructions are obtained using a language model and these rewards are used for error back-propagation. The result is a large improvement in zero-shot translation. As opposed to \citet{N16-1101,johnson17}, dual learning does not involve external pseudo-parallel corpora generation or translation into pivot languages. It should be noted that a variant of this dual learning strategy was used for unsupervised NMT \FIXME{Cite Lample and Artexe's work here} which is inherently a MNMT approach. However Unsupervised NMT is still a new approach and needs further exploration before its capacity for MNMT becomes clear.

% An investigation into why zero-shot NMT does not work well without additional pseudo-parallel corpora revealed that the approaches based on \citet{johnson17} do not learn a perfect universal representation for multiple languages as was previously thought. This prevented the zero shot languages from leveraging shared representations from the resource rich translation directions. \FIXME{This is from that rejected ICLR paper which actually is a good paper. THE MISSING INGREDIENT FOR ZERO-SHOT NEURAL MACHINE TRANSLATION.} As such, this work proposes to force the encoders and decoders to generate representations similar to English via adversarial training. The end result is that zero shot translation performance increases dramatically and its performance matches that of pivot translation.

% Zero shot MNMT models have also shown to be useful for initializing several NLP tasks \cite{DBLP:journals/corr/abs-1809-04686}.

% It can be seen that zero shot translation benefits from monolingual data which can be leveraged by reinforcement learning mechanisms or simply by pseudo parallel corpora generation. Zero shot translation is still growing and lessons from unsueprvised NMT might lead to the development of a MNMT model which is no longer constrained by the lack of parallel data.

% \section{Based on Model Characteristics}
% \subsection{Black box}
% \FIXME{TODO: Raj. Since I have expertize in these methods I will write this.}
% \cite{johnson17}
% \cite{D18-1103}
% \cite{Karakanta2018}

% \subsection{Non black box}
% \cite{DBLP:journals/corr/abs-1811-00498}
% \cite{C18-1263}
% \cite{N16-1101}

% \section{Based on Translation Directions}
% \subsection{1 to many}
% \cite{johnson17}
% \cite{D18-1326}

% \subsection{many to one}
% \cite{johnson17}

% \cite{D18-1103}
% \cite{W18-2711}
% \cite{N16-1004}
% \subsection{many to many}
% \cite{johnson17}
% \cite{D18-1103}

% \section{Translation Scenarios}

% \subsection{Joint Learning}

% \subsection{Fine-tuning}

% \subsection{Zeroshot}

% \subsection{Pivot translation}

% \subsection{multisource}
% \cite{Dabre-MTS2017}
% Insert multisource citations here
% \cite{choi2018improving}

==> pivoting.tex <==
\section{Old Section}
\subsection{Pivoting} \label{sec:pivoting}
\FIXME{clarifying the differences between zero-resource and zero-shot explicitly}
Zero-resource NMT was first explored by \citet{firat16}, where a multiway NMT model was used to translate from Spanish to French using English as a pivot language. This pivoting was done either at run time or during pre-training. 

\vspace{2 mm}
\compactpara{Run-Time Pivoting.} This scenario involves first translating from the source to the pivot language and then from the pivot to the target language as in the initial pivot-language approaches for SMT. \citet{firat16} involved a {\it pipeline} through paths in the multiway model, which first translates from French to English and then from English to Spanish. %Pivoting via a multiway model may be better than pivoting via bilingual models. 
They also experimented with using the intermediate English translation as an additional source for the second stage. Surprisingly, most run-time pivoting approaches do not consider the possibility of n-best pivot language translations which can then be translated into the target language and then be re-ranked. Although this will lead to a large amount of run-time latency it will most certainly lead to better results as it did for sentence-level pivot SMT \cite{utiyama2007}.
% Using the intermediate English translation as an additional source for multi-source translation was rather ineffective.
% As a MNMT model is known to give better English translations as compared to a model trained for a single translation direction, such pivoting can certainly lead to better translation quality as compared to the translations given by pivoting using two unidirectional models. 
% \FIXME{or by forcing the models to learn effective pivot language translations. ATTENTION: not clear} 
% The latter approach requires a small source-target parallel corpus and hence is not truly zero resource. However, both approaches are multilingual because of the coupling of the parameters of the otherwise independent models.

\vspace{2 mm}
\compactpara{Pivoting during Pre-Training.} \citet{firat16b} used the MNMT model to first translate the Spanish side of the training corpus to English which in turn is translated into French. This gives a pseudo-parallel French-Spanish corpus where the source is synthetic and the target is original. The MNMT model is {\it fine tuned on this synthetic data} and this enables direct French to Spanish translation. \REVISE{\citet{Costa-Jussa:2019:CNM:3327969.3312575} showed that pivoting during pre-training performs better than run-time pivoting in Chinese-Catalan translation on the Transformer using Spanish as the pivot language.} \citet{firat16b} also showed that a small clean parallel corpus between French and Spanish can be used for fine tuning and can have the same effect as a pseduo-parallel corpus which is two orders of magnitude larger.
Pivoting models can be improved if they are jointly trained as shown by \citet{ijcai2017-555}. {\it Joint training} was achieved by either forcing the pivot language's embeddings to be similar or maximizing the likelihood
of the cascaded model on a small source-target parallel
corpus.
\citet{P17-1176} proposed {\it teacher-student learning} for pivoting where they first trained a pivot-target NMT model and used it as a teacher to guide the behaviour of a source-target NMT model.

==> zero_shot.tex <==
\subsection{Zero-Shot} \label{sec:zero-shot}
The approaches proposed so far involve pivoting or synthetic corpus generation, which is a slow process due to its two-step nature. It is more interesting, and challenging, to enable translation between a zero-resource pair without explicitly involving a pivot language during decoding or for generating pseudo-parallel corpora. 
%This process of directly training a NMT model for a zero-resource pair is known as zero -shot NMT. 
This scenario is known as {\it zero-shot} NMT.
Zero-shot NMT also requires a pivot language but it is only used during training without the need to generate pseudo-parallel corpora. The three aspects of zero-shot learning for MNMT are as follows:

\vspace{2 mm}
\compactpara{Training.} Zero-shot NMT was first demonstrated by \citet{johnson17}. However, this zero-shot translation method is inferior to pivoting. They showed that the context vectors (from attention) for  unseen language pairs differ from the seen language pairs, possibly explaining the degradation in translation quality.
\citet{DBLP:journals/corr/abs-1811-01389} tried to overcome this limitation by augmenting the training data with the pseudo-parallel unseen pairs generated by iterative application of the same zero-shot translation. 
\citet{arivazhagan2018missing} included explicit language invariance losses in the optimization function to encourage parallel sentences to have the same representation. Al-Shedivat and Parikh \cite{al-shedivat-parikh-2019-consistency} proposed consistency agreement-based training to encourage the model agree on translations into auxiliary languages that do not exist parallel sentences in the parallel corpus.
{\it Reinforcement learning} for zero-shot learning was explored by \citet{DBLP:journals/corr/abs-1805-10338} where the dual learning framework was combined with rewards from language models.

\vspace{2 mm}
\compactpara{Corpus Size.}
Work on translation for Indian languages showed that zero-shot works well only when the training corpora are extremely large \cite{Giulia-MTS2017}. As the corpora for most Indian languages contain fewer than 100k sentences, the zero-shot approach is rather infeasible despite linguistic similarity. \citet{DBLP:journals/corr/abs-1811-01389} confirmed this in the case of European languages where small training corpora were used. \citet{Giulia-MTS2017} also showed that zero-shot translation works well only when the training corpora are large, while \citet{aharoni19} show that massively multilingual models are beneficial for zero-shot translation. 

\vspace{2 mm}
\compactpara{Language Control.} Zero-shot NMT tends to translate into the wrong language at times. This can happen if the internal representations of multiple target languages are too similar despite using the ``target language'' token trick. It is possible to train separate softmaxes for each target language but this merely complicates the model design and thus \citet{DBLP:journals/corr/abs-1711-07893} proposed to filter the output of the softmax so as to force the model to translate into the desired language. This method is rather effective despite its simplicity. Future approaches could consider training models with language masked softmaxes so as to completely prevent any possibility of language mixing.

% \FIXME{@Anoop: how about these paper \cite{DBLP:journals/corr/abs-1805-10338}?}

%A similar work by \citet{DBLP:journals/corr/abs-1711-07893} relied on appending target {\it language tag} per source word but is essentially the same as \citet{johnson17}.
%However, work on translation for Indian languages \cite{Giulia-MTS2017} showed that zero-shot works well only when the training corpora are extremely large. As the corpora for most Indian languages contain fewer than 100k sentences, the zero-shot approach is rather infeasible despite linguistic similarity. \citet{DBLP:journals/corr/abs-1811-01389} confirmed this in the case of European languages where small training corpora were used. 

%Zero-shot NMT models trained in this fashion tends to translate into the wrong language at times and \citet{DBLP:journals/corr/abs-1711-07893} proposed to {\it filter the output} of the softmax so as to force the model to translate into the desired language. They further proposed to incorporate linguistic information such as part-of-speech and morphological features for a {\it factored representation} of the input sentences which led to a further improvement in translation quality. 

% Another important point is that it is better to incorporate multiple translation directions, including redundant directions such as English to English, to improve zero shot translation quality.

% \compactpara{Sophisticated models.}
% This initial success in zero-shot NMT motivated more sophisticated learning-based mechanisms, which have advanced the state-of-art. \citet{P17-1176} proposed {\it teacher-student learning} where they first trained a pivot-target NMT model and used it as a teacher to guide the behaviour of a source-target NMT model.
% The teacher-student method was used in a multi-model fashion by \citet{DBLP:conf/aaai/ChenLL18} where the teacher model is an image captioning model which learns to caption an image into the source language and the student model is the source to target NMT model. 
% {\it Reinforcement learning} for zero-shot learning was explored by \citet{DBLP:journals/corr/abs-1805-10338} where the dual learning framework was combined with rewards from language models. 

